Statistics of spikes trains, synaptic plasticity and Gibbs distributions

We introduce a mathematical framework where the statistics of spikes trains, produced by neural networks evolving under synaptic plasticity, can be analysed.

==> adapt.tex <==
\su{Synaptic adaptation.}
 

In this paper we investigate the effects of synaptic plasticity rules where the characteristic
time scale $T$ is quite a bit larger than the time scale of evolution of the neurons. On practical/numerical  grounds one proceeds as follows.
Neurons are evolving
according to (\ref{DNN}), with a time scale $t$.
We let the neurons evolve over a time windows of width $T$ and records the spikes trains.
Then one update the synaptic weigths according to (\ref{DSyn}). This  has the consequence
of modifying neurons dynamics and possibly spike trains (see discussion below).
In this situation  the synaptic weights update can be written as a function of the 
empirical average  $\pTo(\tomei,\tomej)$ which converges to
the joint probability of the raster plot for the pre- and post-synaptic neuron
as $T \to \infty$. 

As an example we consider slow adaptation rules where the coupled evolution of neurons/synapses writes:

\beq\label{Dcoupled}
\left\{
\baR{ccc}
\VTtp&=&\FgT(\VTt) \\
\WijTp&=&\WijT+  \epsilon g\left(\WijT,\omeit,\omejt)\right)
\eaR
\right.
\eeq

\nid where 

\beq \label{Fgengij}
\baR{ccc}
g(W_{ij},\omeit,\omejt)
\sum_{kl} \hijkl\pTo\left[\aijkl\right].
\eaR
\eeq

\nid with $\omeit=[\omega_i(t-T) \dots \omega_i(t)]$. We use  the notation 
$\omeit^k\times \omejt^l$ for
the finite set of lists $\left\{\omega_i(t_1) \dots \omega_i(t_k) \omega_j(t'_1) \dots \omega_j(t'_l) \right\}, t_1, \dots t_k, t'_1 \dots t'_k, \in [t-T,t]$.
Thus, the term $\gijuu$ accounts for pairs of spikes,
the term $\gijdu$ for triplets of form $\omega_i(t_1)\omega_i(t_2)\omega_j(t'_1)$,
$\dots$. Note that the explicit form of $g$ 
is usually derived from phenomenological considerations
as well as experimental results. These results are usually based
on a repetition of experiments involving the excitation
of pre- and post-synaptic neurons by spike trains. The phenomenological
plasticity rules derived from these experiments are therefore 
of statistical nature.
Note that we keep the notation $\bg$ for the set of parameters, including
the synaptic weights. Thus, $\gT$ is the set of parameters at plasticity epoch
$\tau$. The parameter $\epsilon$ ensures an adiabatic evolution of
the weights (i.e. $\delta \WijT$ is small).\\


\st{Variational formulation.}
Let us now formalize this coupled evolution (\ref{Dcoupled}) in the  context
of thermodynamic formalism. We want to propose a canonical way to describe
the empirical measure evolution when iterating synaptic plasticity rules.
For this we make the assumption that each $\poT$ can be approximated by a Gibbs
measure with potential $\psiT$ and topological pressure $\PT$.
The synaptic update results in a change of parameters $\bg$, $\gTp=\gT+\delta \gT$
where $\delta \gT$ is assumed to be small (this is the role of the constant
$\epsilon$ in (\ref{DSyn})). This induces a variation of the potential
$\psiTp=\psiT+\delta\psiT$ and of the pressure $\PTp=\PT+\delta \PT$.
Note that $\delta\psiT,\delta \PT$ may not be small even if $\delta \gT$ is. 

Consider now a finite range potential $\phi$ of form:
%
%
\beq\label{phiplast}
\phi(\tom;\bl)=\sum_{i,j=1}^N  \lambda_{ij}(W_{ij})\phi_{ij}(\tom)
\eeq
%
%
\nid with:
%
%


\beq
\phi_{ij}(\tom)=\sum_{k,l}  A_{ij}^{(kl)}(\omeitk \times \omejtl) 
\eeq
%
% 
 \nid with $\lambda_{ij}(\WijT)=0$. Then,  from (\ref{moypsi}):
%
%
\beq\label{dPdW}
\left.\frac{\partial P(\psiT + \phi)}{\partial W_{ij}}\right|_{\WijT}=
\sum_{k,l}\nu_{\psiT}\left[ \left. \frac{\partial \lambda_{ij}}{\partial W_{ij}}\right|_{\WijT} A_{ij}^{(kl)}(\omeitk \times \omejtl) \right].
\eeq
%
%
Since $\nu_{\psiT}$ is a statistical model for $\pToT$, setting
%
 
$$\aijkl=\left. \frac{\partial \lambda_{ij}}{\partial W_{ij}}\right|_{\WijT} A_{ij}^{(kl)}(\omeitk \times \omejtl),$$
%
%
provides
an approximation of  $g_{ij}\left[ W_{ij},\pTo(\tomei,\tomej)\right]$  given by (\ref{Fgengij}).

%
%
Thus the adaptation rule (\ref{DSyn}) can be written in the form:
%
%
\beq\label{AdaptRuleVar}
\delta\gT =  \grad P(\psiT + \epsilon \phi)
\eeq
%
% 
\nid where $\phi \equiv \phi(\tom;\bl)$ is given by (\ref{phiplast}) with $\bl \equiv \bl(\bg)$.


==> numex.tex <==


\su{A numerical example.}

\ssu{Model.}

\sssu{Adaptation rule.}

We consider an adaptation rule of type (\ref{STDPFC})
%
$$\WijTp=\lambda \WijT+  \frac{\epsilon}{T} \sum_{t=1}^T \sum_{s=1}^{T} f(s-t)\omeit(s)\omejt(t)=
\lambda \WijT+  \frac{\epsilon}{T} \sum_{t=1}^T \sum_{u=1-t}^{T-t} f(u)\omeit(t+u)\omejt(t),$$
%
where :
%
\beq\label{fSTDP}
f(x)=
\left\{
\baR{lll}
A_- e^{\frac{x}{\tau_-}}, \ x <0;\\
A_+ e^{-\frac{x}{\tau_+}}, \ x >0;\\
0 \ x=0,
\eaR
\right.
\eeq 
%
%
with $A_-<0$ and $A_+>0$.
Since $f(x)$ becomes negligible as soon as $x \gg \tau_+$ or $x \ll -\tau_-$, we
may consider that $f(u) =0$ whenever $|u| > C \deq 2 \max(\tau_+,\tau_-)$.
Moreover, this rule has a particular feature: it enhances LTP for small
$t$ and LTD for large $t$ ($t \sim T$). To avoid this unexpected effect we consider instead
a rule of form:

$$
\WijTp=
\lambda \WijT+  \frac{\epsilon}{T-2C} \sum_{t=C}^{T-C} \omejt(t) \sum_{u=-C}^{C} f(u)\omeit(t+u).
$$
%
Set :

\beq\label{Si}
S_i(\tom)= \sum_{u=-C}^{C} f(u)\omei(u),
\eeq

\nid and:

\beq\label{Hij}
H_{ij}(\tom)=\omega_j(0)S_i(\tom).
\eeq 

Then the adaptation rule writes, in terms of the empirical measure $\pToT$:
%
\beq\label{ruleexp1}
\WijTp=
\lambda \WijT+  \epsilon \frac{T}{T-2C} \pToT\left[H_{ij}\right],
\eeq
%
%
%
Note that $H_{ij}$ is a finite
range potential with range $2C$. One may consider $C \to \infty$ as well,
in which case the corresponding potential is called (? Keller) and behaves
suitably due to the exponential decay of $f(u)$.
As $T \to \infty$ the adaptation rule becomes 

\beq\label{ruleth1}
\WijTp=
\lambda \WijT+  \epsilon \poT\left[H_{ij}\right]= \poT\left[\lambda \WijT+  \epsilon H_{ij}\right].
\eeq

We shall use the rule (\ref{ruleexp1}) for numerical simulation and its limit (\ref{ruleth1}) for theoretical developments.

\sssu{Effects of the adaptation rule on the synaptic weights distribution.}

The only non trivial term in this adaptation rule is the term $S_i(\tom)$ (eq. \ref{Si}),
which can be written, according to the form (\ref{fSTDP}) of $f$:
%
%
$$
S_i(\tom)=A_- \sum_{u=-C}^{-1} e^{\frac{u}{\tau_-}}\omei(u)+
A_+ \sum_{u=1}^C e^{-\frac{u}{\tau_+}}\omei(u).
$$
%
%
It can be either negative, inducing LTD or positive inducing LTP.
In particular, its average with respect to the empirical measure $\poT$ reads:
%
%
$$\poT(S_i)=
A_- r_i(\tau) \sum_{u=-C}^{-1} e^{\frac{u}{\tau_-}}+A_+ r_i(\tau) \sum_{u=1}^C e^{-\frac{u}{\tau_+}},$$
%
%
where $r_i(\tau)=\poT(\omei)$ is the frequency rate of neuron $i$ in the $\tau$-th adaptation epoch. Thus:

\beq \label{PoTSi}
\poT(S_i)=
r_i(\tau) 
\left[
A_- e^{-\frac{1}{\tau_-}}\frac{1-e^{-\frac{C}{\tau_-}}}{1-e^{-\frac{1}{\tau_-}}}
+
A_+ e^{-\frac{1}{\tau_+}}\frac{1-e^{-\frac{C}{\tau_+}}}{1-e^{-\frac{1}{\tau_+}}}.
\right]
\eeq

The term in the brackets neither depends on  $\tom$ nor on $\tau$,
but only on the adaptation rule parameters $A_-,A_+,\tau_-,\tau_+,C$.
This leads us to conjecture the existence of 3 regimes.

\bit
\item\textbf{cooperative regime.} If 
%
$$A_- e^{-\frac{1}{\tau_-}}\frac{1-e^{-\frac{C}{\tau_-}}}{1-e^{-\frac{1}{\tau_-}}}
+
A_+ e^{-\frac{1}{\tau_+}}\frac{1-e^{-\frac{C}{\tau_+}}}{1-e^{-\frac{1}{\tau_+}}}>0$$
%
then $\poT(S_i)>0$. We expect then a tendency for the synaptic weights to become more positive.
Since a weight cannot change its sign the final picture should be positive or zero
synaptic weights. This corresponds to a cooperative system \cite{hirsh:88}. 

\item\textbf{competitive regime.}
On the opposite if

$$A_- e^{-\frac{1}{\tau_-}}\frac{1-e^{-\frac{C}{\tau_-}}}{1-e^{-\frac{1}{\tau_-}}}
+
A_+ e^{-\frac{1}{\tau_+}}\frac{1-e^{-\frac{C}{\tau_+}}}{1-e^{-\frac{1}{\tau_+}}}<0$$

\nid we expect the weights to become  negative or zero.   This corresponds to a competitive system \cite{hirsh:88}. 

\item\textbf{intermediate regime.}

The intermediate regime corresponds to 

$$A_- e^{-\frac{1}{\tau_-}}\frac{1-e^{-\frac{C}{\tau_-}}}{1-e^{-\frac{1}{\tau_-}}}
+
A_+ e^{-\frac{1}{\tau_+}}\frac{1-e^{-\frac{C}{\tau_+}}}{1-e^{-\frac{1}{\tau_+}}}=0$$

\nid where no clear cut tendancy in the synaptic weights evolution should be distinguished.
\eit

\textbf{J.C. A verifier.}
 
\sssu{Dynamical effects of the adaptation rule.}

In the light of the preceeding analysis we conjecture the following effects
of the adpatation on the neuron evolution. 

\bit 

\item \textbf{Cooperative regime.}
In this case, the dynamics to become trivial with neurons firing at each time or
quiescent forever.

\item \textbf{Competitive regime.} Idem ?

\item \textbf{Intermediate regime.} Le plus interessant.

\eit

\textbf{J.C. A verifier.}


\sssu{Statistical effects of the adaptation rule.}

We assume that $\pToT$ converges almost surely toward a Gibbs distribution
$\npT$ with a potential $\psiT$ such that $\poT \equiv \npT$ and a topological pressure
$\PT$. Call $\cH(\tom) \deq \left\{H_{ij}(\tom) \right\}_{i,j=1}^N$ 
Set $\bphi_{\cW}(\tom)=(\lambda -1)\cW+  \epsilon \cH(\tom)$. According to section
\ref{adapt} we may write the adaptation rule (\ref{ruleexp1}) in the form:
%
%
\beq
\dWijT=
\left. 
\frac{\partial P\left[\psiT+ (\cW-\cWT).\bphi_{\cW} \right]}{\partial W_{ij}} 
\right|_{\cW=\cWT}=\npT\left[\bphi \right]
\eeq
%
%
\nid whenever $P$ is differentiable, with $(\cW-\cWT).\bphi_{\cW}=\sum_{i,j=1}^N (\Wij-\WijT) \phi_{ij}$.
In this case, the variation of pressure between epoch $\tau$ and $\tau+1$ is given by:

$$\delta P^{(\tau)} =
\PTp-\PT= P\left[\psiT+ (\cWTp-\cWT).\bphi_{\cW} \right] - \PT $$
%
$$
\sim
\sum_{i,j=1}^N\left.
\frac{\partial P\left[\psiT+ (\cW-\cWT).\bphi_{\cW} \right]}{\partial W_{ij}} 
\right|_{\cW=\cWT} \dWijT
$$

Hence
%
$$
\delta P^{(\tau)} \sim \sum_{i,j=1}^N {\dWijT}^2 >0
$$
%
Therefore the adaptation rule  is a gradient system which tends to maximize the pressure.\\

\textbf{Test J.C. .} Check that the pressure increases with $T$.
\\

An equilibrium point is defined by $\dW=0$ and it corresponds to a maximum of the pressure.
Therefore:
$$\left.\frac{\partial P\left[\psis+ (\cW-\cWs).\bphi \right]}{\partial W_{ij}}\right|_{\cW=\cWs}=\nus\left[\phi_{ij} \right]=0.$$


\nid where $\nus$ is a Gibbs measure with potential $\psis$.
This implies:

\beq
\cW^\ast=\frac{\epsilon}{1-\lambda} \nus\left[\cH \right]
\eeq

This gives, component by component, and making $\cH$ explicit:

\beq
W_{ij}^\ast=\frac{\epsilon}{1-\lambda} \sum_{u=-C}^{C} f(u) \nus\left[ \omej(0) \omei(u)\right],
\eeq

\nid where $\nus\left[ \omej(0) \omei(u)\right]$ is the probability, in the asymptotic regime,
that neuron $i$ fires at time $u$ and neuron $j$ fires at time $0$. Hence the asymptotic synaptic
weights are purely expressed in terms of neurons pairs correlations. \textbf{discuter liens avec Bialek.}\\

\textbf{J.C. Verifier.}\\

Note that  $P(\psis)=\sup_{\nu \in \cM^{inv}_{\bgs}} \left[h(\nu)+\nu(\psis)\right]=h(\nus)+\nus(\psis)$.

\textbf{Conjecture} $\psi^{\ast}=\cH$




